Domain Overlapping Algorithm with Nonlinear Mapping for Collocation-Based Solutions of Eigenvalue Problems

This paper presents four novel domain decomposition algorithms integrated with nonlinear mapping techniques to address collocation-based solutions of eigenvalue problems involving sharp interfaces or steep gradients. The proposed methods leverage the spectral accuracy of Chebyshev polynomials while overcoming limitations of existing tools like Chebfun, particularly in preserving higher-order derivative continuity and enabling flexible node clustering near discontinuities. Key findings include the following: for algorithm Performance: The one-point overlap method demonstrated significant improvements over global mapping approaches, reducing required grid points by orders of magnitude while maintaining spectral convergence. The two-point overlap method further methods generalized the approach, allowing arbitrary node distributions and nonlinear mappings. These achieved exponential error reduction for Burgers equation) by combining Taylor expansions with Chebyshev derivatives in overlap regions. While Chebfun splitting strategy automates domain decomposition, it enforces only C0 continuity, leading to discontinuous higher derivatives. In contrast, the proposed algorithms preserved smoothness up to CN continuity, critical for eigenvalue problems in hydrodynamic stability and nonlinear BVPs. Validation on 3D channel flow with viscosity stratification and Burgers equation highlighted the methods robustness. For instance, eigenvalue calculations for miscible core-annular flows matched prior results while resolving sharp viscosity gradients with fewer nodes.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk --shell-escape -pdf \"$_[0]\"" );
    }
}
